Learning Efficient Policies for Picking Entangled Wire Harnesses: An Approach to Industrial Bin Picking

Wire harnesses are essential connecting components in manufacturing industry but are challenging to be automated in industrial tasks such as bin picking. They are long, flexible and tend to get entangled when randomly placed in a bin. This makes it difficult for the robot to grasp a single one in dense clutter. Besides, training or collecting data in simulation is challenging due to the difficulties in modeling the combination of deformable and rigid components for wire harnesses. In this work, instead of directly lifting wire harnesses, we propose to grasp and extract the target following a circle-like trajectory until it is untangled. We learn a policy from real-world data that can infer grasps and separation actions from visual observation. Our policy enables the robot to efficiently pick and separate entangled wire harnesses by maximizing success rates and reducing execution time. To evaluate our policy, we present a set of real-world experiments on picking wire harnesses. Our policy achieves an overall 84.6% success rate compared with 49.2% in baseline. We also evaluate the effectiveness of our policy under different clutter scenarios using unseen types of wire harnesses. Results suggest that our approach is feasible for handling wire harnesses in industrial bin picking.

==> cover_letter.tex <==
Tamim Asfour, Prof. Ph.D.
Editor-in-Chief
IEEE Robotics and Automation Letters (RA-L)
November 10, 2022

Dear Prof. Tamim Asfour, 
We would like to thank you for accepting our manuscript entitled “Learning Efficient Policies for Picking Entangled Wire Harnesses: An Approach to Industrial Bin Picking”. We would also like to take this opportunity to express our thanks to the Editor and Reviewers for their valuable comments. 

The manuscript has been revised for better readability according to the suggestions. We have carefully corrected the typos and grammar of the manuscript. We again appreciate the kindness of the Editor and Reviewers in helping improve the manuscript. 

Sincerely,

Corresponding Author
Xinyi Zhang
Graduate School of Engineering Science, Osaka University
Machikaneyama 1-3, Toyonaka City, Osaka Pref., Japan
E-mail: xinyiz0931@gmail.com
Tel: +81-6-6850-6383

Additional Contact
Kensuke Harada, Professor
Graduate School of Engineering Science, Osaka University
Machikaneyama 1-3, Toyonaka City, Osaka Pref., Japan
E-mail: harada@sys.es.osaka-u.ac.jp
Tel: +81-6-6850-6380

